Data Augmentation for Conflict and Duplicate Detection in Software Engineering Sentence Pairs

This paper explores the use of text data augmentation techniques to enhance conflict and duplicate detection in software engineering tasks through sentence pair classification. The study adapts generic augmentation techniques such as shuffling, back translation, and paraphrasing and proposes new data augmentation techniques such as Noun-Verb Substitution, target-lemma replacement and Actor-Action Substitution for software requirement texts. A comprehensive empirical analysis is conducted on six software text datasets to identify conflicts and duplicates among sentence pairs. The results demonstrate that data augmentation techniques have a significant impact on the performance of all software pair text datasets. On the other hand, in cases where the datasets are relatively balanced, the use of augmentation techniques may result in a negative effect on the classification performance.

==> Table/augment_sentences.tex <==
\begin{tabular}{l|rrrr|rr}
\toprule
DA Methods & WorldVista & UAV & PURE & OPENCOSS & StackOverflow & Bugzilla\\
\midrule
No DA & 11.66 & 6.00 & 6.66 & 3.33 & 30 & 30 \\
\midrule
Shuffling & 
Back Translation &
Paraphrasing & 
NV-WNS & 
AA-W2V  &
T-WNL &
Combined DA & 

\end{tabular}

==> Table/duplicate_results.tex <==
\begin{tabular}{l p{2cm} l r r r}
\toprule
\textbf{Dataset}&\textbf{\# of Duplicate Instances}&\textbf{DA Technique}&\textbf{Precision}&\textbf{Recall}&\textbf{F1-score} \\
\midrule
 \rowcolor{gray!15}StackOverflow & 180 & No Augmentation &0.875 $\pm$ 0.005 & 0.802 $\pm$ 0.020  & 0.833 $\pm$ 0.013 \\
 & 180 & Paraphrasing &0.889 $\pm$ 0.025 & 0.755 $\pm$ 0.028 & 0.805 $\pm$ 0.015\\
 \cmidrule{2-6}
 \rowcolor{gray!15}& 270 & No Augmentation & 0.909 $\pm$ 0.026 & 0.791 $\pm$ 0.046& 0.835 $\pm$ 0.030 \\
 & 270 & Paraphrasing &0.873 $\pm$ 0.016 & 0.769 $\pm$ 0.016  & 0.811 $\pm$ 0.006 \\
\midrule
 \rowcolor{gray!15} BugZilla & 180 & No Augmentation & 0.903 $\pm$ 0.019 & 0.862 $\pm$ 0.010 & 0.882 $\pm$ 0.010   \\
 & 180 & Shuffling &0.941 $\pm$ 0.012  & 0.845 $\pm$ 0.037 & 0.885 $\pm$ 0.018\\
  \cmidrule{2-6}
 \rowcolor{gray!15}& 270 & No Augmentation & 0.936 $\pm$ 0.004 & 0.901 $\pm$ 0.006 & 0.918 $\pm$ 0.005 \\
 & 270 & Shuffling &0.918 $\pm$ 0.008 &0.873 $\pm$ 0.039 & 0.893 $\pm$ 0.025 \\
\bottomrule

\end{tabular}

==> Table/results_conflict.tex <==
\begin{tabular}{ll|rrr}
     \toprule
      \textbf{Dataset} &\textbf{DA Techniques} & \textbf{Precision} & \textbf{Recall} & \textbf{Macro-F1}  \\
      \midrule
     WorldVista & No Augmentation \citep{malik2022transformer} & & & \\
     
     & Shuffling &   & & \\
     
     & Back Translation  &   & &\\
     
     & Paraphrasing &  & &\\
     & NV-WNS & & &\\
     
     
     &AA-W2V & &&\\
     &T-WNL &&& \\
     
     & Combined DA & & & \\
     
     \midrule
     UAV & No Augmentation \citep{malik2022transformer} & & & \\
     
     & Shuffling &   & & \\
     
     & Back Translation  &   & &\\
     
     & Paraphrasing &  & &\\
     & NV-WNS & & &\\
     
     &AA-W2V & &&\\
     &T-WNL & & & \\
     
     & Combined DA & & & \\
     
     
     
     
     \midrule
     PURE & No Augmentation \citep{malik2022transformer} & & & \\
     
     & Shuffling &   & & \\
     
     & Back Translation  &   & &\\
     
     & Paraphrasing &  & &\\
     & NV-WNS & & &\\
     
     
     &AA-W2V & &&\\
     &T-WNL &&& \\
     
     & Combined DA & & & \\
     
     
     
     
     \midrule
     OPENCOSS & No Augmentation \citep{malik2022transformer} & & & \\
     
     & Shuffling &   & & \\
     
     & Back Translation  &   & &\\
     
     & Paraphrasing &  & &\\
     & NV-WNS & & &\\
     
     
     &AA-W2V & &&\\
     &T-WNL &&& \\
     
     & Combined DA & & & \\
     
     

     
     
     \bottomrule
\end{tabular}

==> Table/results_duplicate.tex <==
\begin{tabular}{ll|rrr}
     \toprule
      \textbf{Dataset} &\textbf{DA Techniques} & \textbf{Precision} & \textbf{Recall} & \textbf{Macro-F1}  \\
      \midrule
     StackOverflow & No Augmentation  & & & \\
     
     & Shuffling & & & \\
     
     & Back Translation  &   & &\\
     
     & Paraphrasing &  & &\\
     & NV-WNS & & &\\
     
     
     &AA-W2V & &&\\
     &T-WNL &&& \\
     
     & Combined DA & & & \\
     
     \midrule
     Bigzilla & No Augmentation  & & & \\
     
     & Shuffling &  & & \\
     
     & Back Translation  &   & &\\
     
     & Paraphrasing &  & &\\
     & NV-WNS & & &\\
     
    
     & Combined DA & & & \\
     \bottomrule
\end{tabular}

==> Table/traditional_DA_sample.tex <==
\begin{tabular}{l p{0.35\textwidth}}
\toprule
\textbf{DA technique} & \textbf{Augmented Sentence} \\
\midrule
Shuffling & \\
Back Translation &  \\
Paraphrasing & Each activated UAV should have a unique ID assigned by the \_ VehicleCore\_.\\

\bottomrule
\end{tabular}
